ALBERT: A Lite BERT for Self-supervised Learning of Language Representations

Increasing model size when pretraining natural language representations often results in improved performance on downstream tasks. However, at some point further model increases become harder due to GPU/TPU memory limitations and longer training times. To address these problems, we present two parameter-reduction techniques to lower memory consumption and increase the training speed of BERT. Comprehensive empirical evidence shows that our proposed methods lead to models that scale much better compared to the original BERT. We also use a self-supervised loss that focuses on modeling inter-sentence coherence, and show it consistently helps downstream tasks with multi-sentence inputs. As a result, our best model establishes new state-of-the-art results on the GLUE, RACE, and \squad benchmarks while having fewer parameters compared to BERT-large. The code and the pretrained models are available at https://github.com/google-research/ALBERT.

==> data.tex <==
% DO NOT WRITE HERE, this content has been moved to the models_experiments.tex file
\section{Experimental Setup}

\subsection{Pretraining}

Following \bert\citep{devlin2018bert}, we use \textsc{BookCorpus}~\citep{zhu2015aligning} and English Wikipedia for pretraining baseline models, which consist of 16GB uncompressed text. In particular, we format input as ``\textsc{[CLS]} $x_1$ \textsc{[SEP]} $x_2$ \textsc{[SEP]}'', where $x_1=x_{1,1},x_{1,2}\cdots$ and $x_2=x_{1,1},x_{1,2}\cdots$ are two segments.\footnote{A segment is usually comprised of more than one natural sentence, which has been shown to benefit performances in \cite{liu2019roberta}.} Unlike \bert, we always limit the maximum input length to be 512 and randomly generate input sequences shorter than 512 with a probability of 10\%. We use a vocabulary size of 30,000, tokenized by SentencePiece~\citep{kudo-richardson-2018-sentencepiece}. For our best model, we also use additional training data from~\cite{liu2019roberta} and~\cite{yang2019xlnet}. When generating masked inputs, we use n-gram masking, similar to~\cite{joshi2019spanbert} where the length of each n-gram mask is selected randomly. The probability for the length $n$ is


\begin{align}
    p(n) &= \frac{1/n}{\sum_1^N{1/k}}
\end{align}

We set the maximum length of n-gram (i.e. $N$) to be 3 as empirically it gives the best performance.

All the models are pretrained with a batch size of 4096 using \textsc{Lamb} optimizer~\citep{you2019reducing}, and the learning rate is set to be 0.00176 ~\citep{you2019reducing}. All of our models are trained 125,000 steps unless specified. 


\subsection{Evaluation}

\subsubsection{Downstream Evaluation}

Following \citep{yang2019xlnet,liu2019roberta}, we evaluate our models on three popular benchmarks: The General Language Understanding Evaluation (GLUE) benchmark~\citep{wang-etal-2018-glue}, The Stanford Question Answering Dataset (\squad;~\citealp{rajpurkar-etal-2016-squad,rajpurkar-etal-2018-know}) and The ReAding Comprehension from Examinations (RACE;~\citealp{lai2017race}). Please see the detailed description of these benechmarks in Appendix \ref{downstream_detailed_description}. Similar to \cite{liu2019roberta}, we perform early stopping on the development sets.

\subsubsection{Intrinsic Evaluation}

To monitor the training progress, we create a development set based on the development sets from \squad and RACE. We follow the same procedures that we use for creating training set. We report accuracies for both masked LM and sentence classification tasks. 

==> models.tex <==
% DO NOT WRITE HERE, this content has been moved to the models_experiments.tex file 
\section{ALBERT}
In this section, we present a set of ALBERT models and give an overall comparison of these models to the original BERT models. 
We will have detailed analysis of how each component contribute to the differences and the reasons behind the choices of these models in section \ref{sec:experiments}.

\subsection{Model architectures}
BERT uses the popular transformer encoder architecture \citep{vaswani2017attention}, which we will not review in detail. Following the annotation of BERTs,
we denote the number transformer encoder layers as $L$, the hidden size as $H$, the number of self-attention heads as $A$,
and the vocab embedding size as $E$. We also set the feed-forward/filter size to be $4H$. We primary report results on the models listed in Table \ref{table:model_architecture}. 
The major differences between BERT and ALBERT are smaller vocabulary embedding size and cross-layer parameter sharing. Because of these two techniques, ALBERTs have much smaller parameter size compared to BERT with similar architecture. For example, ALBERT-large has about 18x less parameters compared to BERT-large. For BERTs, besides base and large models as reported by \cite{devlin2018bert}, we are able to train an xlarge model with a hidden size 2x as large as the BERT-large model. However, this BERT-xlarge has about 1.3 billions parameters, which make it difficult to train as it requires a Cloud-TPU machine with 1024 chips that is hard to get. On the contrary, ALBERTs have much smaller parameter size hence memory footprint, so we are able to scale to a model with 4x larger hidden size than BERT-large while having smaller parameter size. 




\begin{table}
\small
\centering
\begin{tabular}{l  l | c c c c c c}
 \multicolumn{2}{c}{Model}  &Parameters	&Layers	&Hidden	& Heads	&Embedding &Parameter-sharing \\
\hline
\multirow{3}{*}{BERT}    &base	        &110M    &12 & 768  & 12 & 768 & False\\
    &large	        &340M	 &24 & 1024 & 16 & 1024 & False\\
    &xlarge	&1370M	 &24 & 2048 & 32 & 2048 & False\\
    \hline
\multirow{4}{*}{ALBERT}    &base	        &12M     &12 & 768  & 12 & 128 & True \\
    &large	        &18M	 &24 & 1024 & 16 & 128 & True\\
    &xlarge	&59M	 &24 & 2048 & 32 & 128 & True\\
    &xxlarge	&233M	 &12 & 4096 & 64 & 128 & True\\
\end{tabular}
\caption{The architectures of the primary models reported in this paper.}
\label{table:model_architecture}
\end{table}


\subsection{Overall Performance Comparison}
\label{overall-performance}

\begin{table}
\small
\centering
\begin{tabular}{ l l | c  c c c c c c}
 \multicolumn{2}{c}{Model}            	&SQuAD1.1	&SQuAD2.0	&MNLI-m	&SST-2	&RACE	&Avg & Speedup\\
\hline
\multirow{3}{*}{BERT} &base	          &90.5/83.3	&80.3/77.3	&84.1	&91.7	&68.3	&82.1 & 17.7x \\

    &large	        	&92.4/85.8	&83.9/80.8	&85.8	&92.2	&73.8	&85.1 & 3.8x\\
    &xlarge		&86.3/77.9	&73.8/70.5	&80.5	&87.8	&39.7	&76.7 & 1.0\\
\hline 
\multirow{4}{*}{ALBERT}  &base	        	    &89.3/82.1	&79.1/76.1	&81.9	&89.4	&63.5	&80.1 &21.1x \\
&large	        	    &90.9/84.1	&82.1/79.0	&83.8	&90.6	&68.4	&82.4 &6.5x\\
&xlarge		    &93.0/86.5	&85.9/83.1	&85.4	&91.9	&73.9	&85.5 & 2.4x\\
&xxlarge		& \textbf{94.1/88.3}	&\textbf{88.1/85.1}	&\textbf{88.0}	&\textbf{95.2}	&\textbf{82.3}	&\textbf{88.7} & 1.2x\\
\end{tabular}
\caption{Dev sets results for primary models pre-trained over BookCorpus and Wikipedia for 125k steps. The average score are averaged over the representative downstream tasks. For SQuAD datasets, the two metrics are first averaged.}
\label{table:overall_comparison}
\end{table}



We compare the performance of the primary models listed in Table \ref{table:overall_comparison} on the dev sets of several representative downstream tasks including SQuAD v1.1, SQuaAD v2.0, MNLI-m, SST-2 and RACE tasks. We first observe that BERT-xlarge gets significantly worse results than BERT-base on all metrics. This indicates that a model like BERT-xlarge is more difficult to train than those that have smaller parameter sizes. 
Another interesting observation we have is the speed of data throughput. The slowest one is the BERT-xlarge model, which we use as the baseline. ALBERT models have higher data throughput than their corresponding BERT models. As the model get larger, the differences between a BERT model and its light version become bigger. A ALBERT xlarge can be trained about 2.4x faster than BERT-x large. The 12-layer ALBERT-xxlarge model outperform all other models significantly. Compared to BERT-large, which has roughly 1.45x more parameters, ALBERT-xxlarge has an average of $3.6\%$ absolute improvements over 5 downstream tasks and $8.5\%$ absolute improvements over the RACE task. 

